Pseudoscalar Higgs boson decay to three parton amplitudes at NNLO to higher orders in the dimensional regulator

We present for the first time the second-order corrections of pseudo-scalar($A$) Higgs decay to three parton to higher orders in the dimensional regulator. We compute the one and two-loop amplitudes for processes, $A\to ggg$ and $A\to q\bar{q}g$ in the effective theory framework. With suitable crossing of the external momenta, these calculations are well-suited for predicting the differential distribution of pseudo-scalar Higgs in association with a jet at hadron colliders, up to next-to-next-to-leading order (NNLO) in the strong coupling constant. These results expanded to higher orders in dimensional regulator will contribute to the full three loop cross section. We implement the finite pieces of the amplitudes in a numerical code which can be used with any Monte Carlo phase space generator.

==> ancillary/Ato3jet/Makefile <==
# ----------------------------------------------------------------------
FC=gfortran

#PATH of handyG
#HANDYG= <<Installation-Path-of-handyG>>
HANDYG=/home/chinmoy/Work/Packages/Source/handyG/install_quad
FFLAGS= -I$(HANDYG)/include -L$(HANDYG)/lib -lhandyg

SRC_DIR=src
OBJ_DIR=obj
BIN_DIR=bin

src= $(wildcard $(SRC_DIR)/*.f95)
obj= $(patsubst $(SRC_DIR)/%.f95,$(OBJ_DIR)/%.o,$(src))

EXEC = Ato3jet

all: $(EXEC)

$(OBJ_DIR)/%.o: $(SRC_DIR)/%.f95
	$(FC) -c $(FFLAGS) $< 
	@for file in $<; do \
		base=`basename $$file .f95`; \
		mv $$base.o $(OBJ_DIR)/$$base.o; \
	done 

Ato3jet: $(obj)
	$(FC) -o $@ $(obj) $(FFLAGS) 
	mv Ato3jet $(BIN_DIR)/

clean:
	-rm -f *.o $(OBJ_DIR)/*.o $(BIN_DIR)/$(EXEC)

# ----------------------------------------------------------------------


==> ancillary/Ato3jet/README <==
************************************************************************************************************************************************
*                    Pseudo-scalar Higgs decay to three parton amplitudes at NNLO to higher orders in dimensional regulator                    *
*						                                                                                               *
*                                                                  A -> j j j                                                                  *
*                                                                                                                                              *
*                                           Pulak Banerjee, Chinmoy Dey, M.C. Kumar and V. Ravindran                                           *
*                                                                                                                                              *
*  For any questions or comments, please contact:  pulak.banerjee@lnf.infn.it, d.chinmoy@iitg.ac.in, mckumar@iitg.ac.in, ravindra@imsc.res.in  * 
************************************************************************************************************************************************

arXiv:2411.XXXX

Requirements: gcc compiler and handyG
----------------------------------------------------------------------------------------------------------
Please give the installation path of handyG in the Makefile, under the variable HANDYG.
----------------------------------------------------------------------------------------------------------

Installation:
----------------------------------------------------------------------------------------------------------

You can also install handyG from the git repository:

`git clone https://gitlab.com/mule-tools/handyg
cd handyG
./configure --prefix= <<Installation-Path-of-handyG>> 
make && make check && make install`
----------------------------------------------------------------------------------------------------------

Compilation:
----------------------------------------------------------------------------------------------------------
After adding the handyG installation path in Makefile please run:

`make -j<n>`
where n represents how many jobs the user wants to run in parallel mode. 

The executable 'Ato3jet' can be found under /bin.
----------------------------------------------------------------------------------------------------------

Running the code:
----------------------------------------------------------------------------------------------------------
The user can change the parameters in the input.input file. PROCESS ID represents the  matrix elements and 
the correspoding powers in \epsilon that the user can choose to run. The PROCESS ID's are as follows: 

------------------------------------------------------------------
Process ID 	Process    Perturbative order       Power of eps
------------------------------------------------------------------
   10		 A2ggg		  1		          0
   11		 A2ggg		  1		          1
   12		 A2ggg		  1		          2
   13		 A2ggg		  1		          3
   14		 A2ggg		  1		          4
   15		 A2qQg		  1		          0
   16		 A2qQg		  1		          1
   17		 A2qQg		  1		          2
   18		 A2qQg		  1		          3
   19		 A2qQg		  1		          4
   20		 A2ggg		  2		          0
   21		 A2ggg		  2		          1
   22		 A2ggg		  2		          2
   23		 A2qQg		  2		          0
   24		 A2qQg		  2		          1
   25		 A2qQg		  2		          2
------------------------------------------------------------------


The user can give their own choice of phase space points, in terms of y and z. Here we have provided 100 
phase space points for the two regions that we discuss in our paper:

1. phasespace_I.input
2. phasespace_II.input

If you want to check the code, please rename the above files to phasespace.input to run the code.

Finally run this code by:
`./bin/Ato3jet`

The output of the runs will be generated inside the output folder.


